Model Predictive Control of a Food Production Unit: A Case Study for Lettuce Production

Plant factories with artificial light are widely researched for food production in a controlled environment. For such control tasks, models of the energy and resource exchange in the production unit as well as those of the plant's growth process may be used. To achieve minimal operation cost, optimal control strategies can be applied to the system, taking into account the availability of resources by control reference specification. A particular advantage of model predictive control (MPC) is the incorporation of constraints that comply with actuator limitations and general plant growth conditions. In this work, a model of a production unit is derived including a description of the relation between the actuators' electrical signals and the input values to the model. Furthermore, a preliminary model based state tracking control is evaluated for production unit containing Lettuce. It could be observed that the controller is capable to track the reference while satisfying the constraint under changing weather conditions and resource availability.

==> ACSD-preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ACSD %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Packages
\usepackage{xspace}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{makecell}
\usepackage{cite}
\usepackage{nicefrac}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsthm}

%%%% Arrows
\newcommand{\ra}{\rightarrow}
\newcommand{\rra}{\rightrightarrows}
\newcommand{\la}{\leftarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\LRa}{\LeftRightarrow}

%%%% Theorems
%\newtheorem{dfn}{Definition}
%\newtheorem{asm}{Assumption}
%\newtheorem{fct}{Fact}
%\newtheorem*{fct*}{Fact}
%\newtheorem{prp}{Proposition}
%\newtheorem*{prp*}{Proposition}
%\newtheorem{lem}{Lemma}
%\newtheorem*{lem*}{Lemma}
%\newtheorem{thm}{Theorem}
%\newtheorem{crl}{Corollary}
%\newtheorem*{crl*}{Corollary}
%\newtheorem{rem}{Remark}
%\newtheorem*{rem*}{Remark}
%\newtheorem{exm}{Example}
%\newtheorem*{exm*}{Example}
%\newtheorem{prb}{Problem}
%\newtheorem*{prb*}{Problem}

%%%% Abbreviations
\newcommand{\ie}{\unskip, i.\,e.,\xspace}
\newcommand{\eg}{\unskip, e.\,g.,\xspace}
\newcommand{\pd}{p.\,d.\xspace}
\newcommand{\sut}{\text{s.\,t.\,}}
\newcommand{\wrt}{w.\,r.\,t.\xspace}
\newcommand{\rt}{r.\,t.\xspace}

%%%% Sets
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}

\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\X}{\ensuremath{\mathbb{X}}}
\newcommand{\Y}{\ensuremath{\mathbb{Y}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\U}{\ensuremath{\mathbb{U}}}

\newcommand{\sm}{\ensuremath{\setminus}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

%%%% Texts
\newcommand{\diam}{\ensuremath{\text{diam}}}
\newcommand{\dom}{\ensuremath{\text{dom}}}
\newcommand{\sgn}{\ensuremath{\text{sgn}}}
\newcommand{\co}{\ensuremath{\text{co}}}
\newcommand{\cco}{\ensuremath{\overline{\text{co}}}}

%%%% Fonts
\newcommand{\bb}[1]{\textbf{#1}}
\newcommand{\ii}[1]{\textit{#1}}
\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}

%%%% Symbols
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\pdiff}[2]{ \ensuremath{ \frac{\partial {#1}}{\partial {#2}} } }
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\newcommand{\ball}{\ensuremath{\mathcal B}}
\newcommand{\tp}{^{\top}}			% Transpose
\newcommand{\D}{\ensuremath{\mathcal{D}}}		% Generalized derivative
\newcommand{\K}{\ensuremath{\mathcal{K}}\xspace}		% Capital kappa
\newcommand{\KL}{\ensuremath{\mathcal{KL}}\xspace}		% Kappa-ell
\newcommand{\Kinf}{\ensuremath{\mathcal{K}_{\infty}}\xspace}		% Kappa-infinity
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\argsup}{arg\,sup}

%%%% References
\newcommand{\reffig}[1]{Fig.\,\ref{#1}}  
%\newcommand{\refFig}[1]{Figure\, \ref{#1}} 

%%%% Wraps
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\scal}[1]{\left\langle#1\right\rangle}

%%%% Probability
\newcommand{\PP}{\ensuremath{\mathbb{P}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}

%%%% Review
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}
\newcommand{\green}[1]{\textcolor{dgreen}{#1}}

%%%% Miscellaneous
\newcommand{\spc}{\ensuremath{\,\,}}	% Logical formula separator

%%%% Environments
\makeatletter
\newcommand{\subalign}[1]{%
	\vcenter{%
		\Let@ \restore@math@cr \default@tag
		\baselineskip\fontdimen10 \scriptfont\tw@
		\advance\baselineskip\fontdimen12 \scriptfont\tw@
		\lineskip\thr@@\fontdimen8 \scriptfont\thr@@
		\lineskiplimit\lineskip
		\ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\crcr
			#1\crcr
		}%
	}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> production_chamber.tex <==
\begin{table}[h]
	\centering	
	\begin{tabular}{lll}
		\hline
		Symbol                     & Description                                & Unit                           \\ \hline
		$T$                        & temperature of air inside chamber          & [\si{\celsius}]                \\
		$C$                        & CO$_2$ concentration of air inside chamber & [\si{\kilogram\meter}$^{-3}$]  \\
		$H$                        & absolute humidity of the air inside        & [\si{\kilogram\meter}$^{-3}$]  \\
		$W_\mathrm{sto}$           & total water in the storage tank            & [\si{\kilogram}]               \\
		$W_\mathrm{med}$           & total water in the growing medium          & [\si{\kilogram}]               \\
		$W_\mathrm{ovf}$           & total water overflowing                    & [\si{\kilogram}]               \\
		$B$                        & biomass/dry matter content of the crop     & [\si{\kilogram\meter}$^{-2}$]  \\
		$u_\mathrm{T}$             & TEC input                                  & [-]                            \\
		$u_\mathrm{V}$             & ventilator input                           & [-]                            \\
		$u_\mathrm{H}$             & humidifier input                           & [-]                            \\
		$u_\mathrm{W1}$            & storage tank pump input                    & [-]                            \\
		$u_\mathrm{W2}$            & growing medium pump input                  & [-]                            \\
		$u_\mathrm{W3}$            & reclaimer pump input                       & [-]                            \\
		$u_{\mathrm{I}i}$          & light input of $i^\mathrm{th}$ LED channel & [-]                            \\
		$T_\mathrm{out}$           & temperature of outside air                 & [\si{\celsius}]                \\
		$C_\mathrm{out}$           & CO$_2$ concentration of outside air        & [\si{\kilogram\meter}$^{-3}$]  \\
		$H_\mathrm{out}$           & absolute humidity of outside air           & [\si{\kilogram\meter}$^{-3}$]  \\
		$\phi_{\mathrm{Q_{TEC}}}$  & heat produced/removed by TEC               & [\si{\joule\second}$^{-1}$]    \\
		$\phi_{\mathrm{Q_{LED}}}$  & heat produced by LEDs                      & [\si{\joule\second}$^{-1}$]    \\
		$\phi_{\mathrm{Q_{evap}}}$ & heat lost due to plant transpiration       & [\si{\joule\second}$^{-1}$]    \\
		$\phi_{\mathrm{Q_{cond}}}$ & heat released due to condensation on walls & [\si{\joule\second}$^{-1}$]    \\
		$\phi_{\mathrm{C_{c\_p}}}$ & gross CO$_2$ consumed by plant             & [\si{\kilogram\second}$^{-1}$] \\
		$\phi_{\mathrm{C_{p\_c}}}$ & gross CO$_2$ produced by plant             & [\si{\kilogram\second}$^{-1}$] \\
		$\phi_{\mathrm{W_{evap}}}$ & water evaporated from plant                & [\si{\kilogram\second}$^{-1}$] \\
		$\phi_{\mathrm{W_{cond}}}$ & water condensed on the chamber walls       & [\si{\kilogram\second}$^{-1}$] \\
		$\phi_{\mathrm{W_{TEC}}}$  & water condensed on the TEC condenser       & [\si{\kilogram\second}$^{-1}$] \\
		$\phi_{\mathrm{W2o}}$      & water overflowing from the storage tank    & [\si{\kilogram\second}$^{-1}$] \\
		$\phi_{\mathrm{W1o}}$      & water overflowing from growing medium      & [\si{\kilogram\second}$^{-1}$] \\ \hline
	\end{tabular}
	\caption{List of symbols used}
\end{table}
\section{Growth Chamber and Plant model}\label{sec:model}
A prototype version of a container farm was developed in a scale comparable to a standard commercial growth chamber to serve as a test-bench. The designed chamber is integrated with various sensors and actuators to facilitate the regulation of climate inside the chamber and resource exchanges. The process model of the designed container is presented in Fig.~\ref{fig:growth_chamber} highlighting the actuator-sensor infrastructure and various energy and resource fluxes. 
Although several actuators are in place, controllability in the state space is restricted by limitations of the actuators and the influence of the external environment.
One such limitation being the cooling capacity of the thermoelectric cooler (TEC).

\begin{figure*}[h]
	\begin{center}
		%\includegraphics[width=13cm]{gfx/Plant_process_growth_chamber_ext}    % The printed column width is 8.4 cm.
		%		\resizebox{\linewidth}{!}{\input{./gfx/Plant_process_growth_chamber_ext.pdf_tex}}
		\def\svgwidth{\linewidth}
		\fontsize{7.5}{8}\selectfont
		\input{./gfx/Plant_process_growth_chamber.pdf_tex}
		\caption{Process model of the system: Container with sensors (S1-S5), air pumps (M1-M2), water pumps (M3-M5), air conditioning unit (thermoelectric cooler based for heating, cooling, condensation), humidifier, LED lighting and the corresponding system states and some of the resource fluxes.} 
		\label{fig:growth_chamber}
	\end{center}
\end{figure*}


A detailed dynamic model and the corresponding parameters of this production chamber is presented in \red{ref COMPAG paper}. A dynamic growth model of Lettuce presented in \citep{book:975318}, and more elaborately in \citep{STRATEN2011}, is used as the subject of interest growing in the chamber. This model considers the effect of light, temperature and CO$_2$ concentrations on the lettuce growth however ignores the effects of day-night light cycles. Equations governing the system states and the resource flux terms are presented in this section to summarize the system under consideration. %A dynamic model of the container with lettuce as presented in this section will be the system under study.

%\begin{strip}
%\begin{subequations}
%	\begin{align}
%	%dB/dt
%	\frac{\mathrm{d}B}{\mathrm{d}t} 
%	&=k_\mathrm{\alpha,\beta} \underbrace{\left(1-e^{-k_{\mathrm{L}}B}\right)
%	\left(\frac{k_\mathrm{I,p}I(-k_\mathrm{p,1}T^2 + k_\mathrm{p,2}T -	k_\mathrm{p,3})(C - k_\mathrm{\Gamma,p})}
%	{k_\mathrm{I,p}I + (-k_\mathrm{p,1}T^2 + k_\mathrm{p,2}T - k_\mathrm{p,3})(C - k_\mathrm{\Gamma,p})} \right)}_{\phi_{\mathrm{C_{c\_p}}}}
%	- k_\mathrm{B_{p\_c}}\underbrace{Bk_\mathrm{Qresp}^{(0.1T - 2.5)}}_{\phi_{\mathrm{C_{p\_c}}}}\\
%	\label{eq:dB/dt}
%	%dT/dt 
%	k_\mathrm{C}\frac{\mathrm{d}T}{\mathrm{d}t}
%	&= \left(T_\mathrm{out}-T\right)k_\mathrm{u_{V}}u_\mathrm{V}
%	+ k_\mathrm{loss}\left(T_\mathrm{out}-T\right)
%- \left(k_\mathrm{l,1} - k_\mathrm{l,2}T\right)\underbrace{\left(1-e^{-k_{\mathrm{L}}B}\right) k_\mathrm{H,p\_c} \left(\frac{k_\mathrm{Hs,1}}{k_\mathrm{R,W}(T+273)} e^{\left(\frac{k_\mathrm{Hs,2}T}{T+k_\mathrm{Hs,3}}\right)}- H\right)}_{\phi_\mathrm{W_{evap}}}\\
%	&+ \left(\frac{k_\mathrm{l,1} - k_\mathrm{l,2}T}{k_\mathrm{l,\epsilon} +1}\right)\underbrace{k_\mathrm{cond}\max\left( \left(H -\frac{k_\mathrm{H}}{(T_\mathrm{c}+273)}
%		e^{\left(\frac{k_\mathrm{Hs,2}T_\mathrm{c}}{T_\mathrm{c}+k_\mathrm{Hs,3}}\right)}\right),0 \right)}_{\phi_\mathrm{W_{cond}}}
%	+ \underbrace{\left(\frac{k_\mathrm{\alpha_q} k_\mathrm{V,max}  u_\mathrm{T} T}{k_\mathrm{R_q}} 
%		+ \frac{{(k_\mathrm{V,max}u_\mathrm{T})}^2} {2k_\mathrm{R_q}}\right)}_{\phi_{\mathrm{Q_{TEC}}}}
%		+ \underbrace{\sum_{i=1}^{4}k_{\mathrm{Q,I}i}u_{\mathrm{I}i}}_{\phi_{\mathrm{Q_{LED}}}}
%	\\
%	\label{eq:dT/dt_full}
%	%dC/dt 
%	k_\mathrm{V}\frac{\mathrm{d}C}{\mathrm{d}t}
%	&=(C_\mathrm{out}-C)k_\mathrm{u_{V}}u_\mathrm{V}
%	- (C_\mathrm{out}-C)k_\mathrm{leak}
%	+ k_\mathrm{C_{p\_c}} \phi_{\mathrm{C_{p\_c}}}
%	- \phi_{\mathrm{C_{c\_p}}}\\
%	\label{eq:dC/dt_full}
%	%dH/dt 
%	k_\mathrm{V}\frac{\mathrm{d}H}{\mathrm{d}t}
%	&= k_\mathrm{u_H}u_\mathrm{H}
%	+ (H_\mathrm{out} - H)k_\mathrm{u_{V}}u_\mathrm{V}
%	+ \phi_\mathrm{W_{evap}}
%	- \phi_\mathrm{W_{cond}}
%	- \phi_\mathrm{W_{TEC}}\\
%	\label{eq:dH/dt_full}
%	%dWsto/dt 
%	\frac{\mathrm{d}W_\mathrm{sto}}{\mathrm{d}t} 
%	&= k_\mathrm{u_W}u_\mathrm{W1} 
%	- k_\mathrm{u_H}u_\mathrm{H}
%	+ \phi_\mathrm{W_{TEC}}
%	- \phi_\mathrm{W1o}\\
%	\label{eq:dW_sto/dt_full}
%	%dWmed/dt 
%	\frac{\mathrm{d}W_\mathrm{med}}{\mathrm{d}t} 
%	&= k_\mathrm{u_W}u_\mathrm{W2}
%	- \phi_\mathrm{W_{evap}}
%	- (1-k_\mathrm{f})\dot{B}
%	- \phi_\mathrm{W2o}\\
%	\label{eq:dW_med/dt_full}
%	%dWovf/dt 
%	\frac{\mathrm{d}W_\mathrm{ovf}}{\mathrm{d}t}
%	&= \phi_\mathrm{W1o}
%	+ \phi_\mathrm{W2o}
%	- k_\mathrm{u_W}u_\mathrm{W3}
%	+ \phi_\mathrm{W_{cond}}\\
%	\label{eq:dW_ovf/dt}
%	\end{align}
%\end{subequations}
%\end{strip}

The two major resource dynamics addressed by the lettuce plant model are the CO$_2$ and water which is consumed and converted into plant biomass $B$. The rate of consumption and production of these resources due to respiration (\ref{eq:phi_Cout}), photosynthesis (\ref{eq:phi_Cin}), and transpiration (\ref{eq:phi_W_evap}) are given as below:
\begin{subequations}\label{eq:phi_humidity}
	\begin{align}
	\begin{split}
	\phi_\mathrm{C_{p\_c}}
	&=Bk_\mathrm{Qresp}^{(0.1T - 2.5)}
	\label{eq:phi_Cout}
	\end{split}\\
	\begin{split}
	\phi_\mathrm{C_{c\_p}}
	&= \left(1-e^{-k_{\mathrm{L}}B}\right)\\
	&\left(\frac{k_\mathrm{I,p}I(-k_\mathrm{p,1}T^2 + k_\mathrm{p,2}T -	k_\mathrm{p,3})(C - k_\mathrm{\Gamma,p})}
	{k_\mathrm{I,p}I + (-k_\mathrm{p,1}T^2 + k_\mathrm{p,2}T - k_\mathrm{p,3})(C - k_\mathrm{\Gamma,p})} \right)
	\label{eq:phi_Cin}
	\end{split}\\
	\begin{split}
	\phi_\mathrm{W_{evap}}
	&= k_\mathrm{H,p\_c} \left(1-e^{-k_{\mathrm{L}}B}\right) \\
	&\left(\frac{k_\mathrm{Hs,1}}{k_\mathrm{R,W}(T+273)} e^{\left(\frac{k_\mathrm{Hs,2}T}{T+k_\mathrm{Hs,3}}\right)} - H\right)
	\label{eq:phi_W_evap}
	\end{split}
	\end{align}
\end{subequations}
 with $I = \sum_{i=1}^{4}k_{\mathrm{u,I}i}u_{\mathrm{I}i}$ being the total light incident on the plant canopy.

Some of the flux components corresponding to heat \eqref{eq:phi_heat}, water vapor \eqref{eq:phi_humidity} and water \eqref{eq:phi_water} flux contributed by chamber and its actuators are given as functions of one of more states or inputs
	\begin{subequations}\label{eq:phi_water}
	\begin{align}
	\begin{split}
	\phi_\mathrm{W1o}
	&= \begin{cases} 
	0       					& \text{if } W_\mathrm{med} \leq k_\mathrm{W1m} \\
	k_\mathrm{u_W}u_\mathrm{W1} 
	- k_\mathrm{u_H}u_\mathrm{H}
	+ \phi_\mathrm{W_{TEC}}      & \text{if } W_\mathrm{med} > k_\mathrm{W1m} \\
	\end{cases}
	\label{eq:phi_W1o}
	\end{split}\\
	\begin{split}
	\phi_\mathrm{W2o}
	&= \begin{cases} 
	0       					& \text{if } W_\mathrm{sto} \leq k_\mathrm{W2m} \\
	k_\mathrm{u_W}u_\mathrm{W2}
	- \phi_\mathrm{W_{evap}}
	- (1-k_\mathrm{f})\dot{B}      & \text{if } W_\mathrm{sto} > k_\mathrm{W2m} \\
	\end{cases}
	\label{eq:phi_W2o}
	\end{split}
	\end{align}
\end{subequations}

\begin{subequations}\label{eq:phi_heat}
	\begin{align}
	\begin{split}
	%Q_LED
	\phi_{\mathrm{Q_{LED}}}
	&=\sum_{i=1}^{4}k_{\mathrm{Q,I}i}u_{\mathrm{I}i}
	\label{eq:phi_Q_LED}
	\end{split}\\	
	\begin{split}
	%Q_TEC
	\phi_{\mathrm{Q_{TEC}}}
	&=\frac{k_\mathrm{\alpha_q} k_\mathrm{V,max}  u_\mathrm{T} T}{k_\mathrm{R_q}} 
	+ \frac{{(k_\mathrm{V,max}u_\mathrm{T})}^2} {2k_\mathrm{R_q}}
	\label{eq:phi_Q_TEC}
	\end{split}\\
	\begin{split}
	\phi_\mathrm{W_{cond}}
	&= \max\left(
	k_\mathrm{cond} \left(H -\frac{k_\mathrm{H}}{(T_\mathrm{c}+273)}
	e^{\left(\frac{k_\mathrm{Hs,2}T_\mathrm{c}}{T_\mathrm{c}+k_\mathrm{Hs,3}}\right)}
	\right),0 \right)
	\label{eq:phi_W_cond}
	\end{split}\\
	\begin{split}
	\phi_\mathrm{W_{TEC}}
	&= \max\left(
	k_\mathrm{TEC}
	\left(H - \frac{k_\mathrm{H}}{(T_\mathrm{q}+273)}
	e^{\left(\frac{k_\mathrm{Hs,2}T_\mathrm{q}}{T_\mathrm{q}+k_\mathrm{Hs,3}}\right)}
	\right),0
	\right)
	\label{eq:phi_W_TEC}
	\end{split}
	\end{align}
	\end{subequations}
where $ T_\mathrm{c} = 0.5(T +T_\mathrm{out})$ is the temperature on the inner surface of the chamber and $T_\mathrm{q}
= T + \left(\frac{\phi_{\mathrm{Q_{TEC}}}}{k_\mathrm{cm}}\right)$ is the temperature on the condenser surface.

The consolidated equations (\ref{eq:dT/dt_full} to \ref{eq:dB/dt}) representing the complete system under study is given by the following:
\begin{subequations} \label{eq:system}
\begin{align}
%dT/dt 
\begin{split}
k_\mathrm{C}\frac{\mathrm{d}T}{\mathrm{d}t}
&= k_\mathrm{u_{V}}\left(T_\mathrm{out}-T\right)u_\mathrm{V}
+ k_\mathrm{loss}\left(T_\mathrm{out}-T\right)\\
&+ \phi_{\mathrm{Q_{TEC}}} + \phi_{\mathrm{Q_{LED}}}%\\
% &- \left(k_\mathrm{l,1} - k_\mathrm{l,2}T\right)\phi_\mathrm{W_{evap}}
%+ \left(\frac{k_\mathrm{l,1} - k_\mathrm{l,2}T}{k_\mathrm{l,\epsilon} +1}\right)\phi_\mathrm{W_{cond}}
\label{eq:dT/dt_full}
\end{split}\\
\begin{split}
%dC/dt 
k_\mathrm{V}\frac{\mathrm{d}C}{\mathrm{d}t}
&=(C_\mathrm{out}-C)k_\mathrm{u_{V}}u_\mathrm{V}
- (C_\mathrm{out}-C)k_\mathrm{leak}\\
&+ k_\mathrm{C_{p\_c}} 	\phi_\mathrm{C_{p\_c}}
- \phi_\mathrm{C_{c\_p}}
\label{eq:dC/dt_full}
\end{split}\\
\begin{split}
%dH/dt 
k_\mathrm{V}\frac{\mathrm{d}H}{\mathrm{d}t}
&= k_\mathrm{u_H}u_\mathrm{H}
+ (H_\mathrm{out} - H)k_\mathrm{u_{V}}u_\mathrm{V}
+ \phi_\mathrm{W_{evap}}\\
&- \phi_\mathrm{W_{cond}}
- \phi_\mathrm{W_{TEC}}\label{eq:dH/dt_full}
\end{split}\\
\begin{split}
%dWsto/dt 
\frac{\mathrm{d}W_\mathrm{sto}}{\mathrm{d}t} 
&= k_\mathrm{u_W}u_\mathrm{W2} 
- k_\mathrm{u_H}u_\mathrm{H}
+ \phi_\mathrm{W_{TEC}}
- \phi_\mathrm{W1o}\label{eq:dW_sto/dt_full}
\end{split}\\
\begin{split}
%dWmed/dt 
\frac{\mathrm{d}W_\mathrm{med}}{\mathrm{d}t} 
&= k_\mathrm{u_W}u_\mathrm{W1}
- \phi_\mathrm{W_{evap}}
- k_\mathrm{fw}\dot{B}
- \phi_\mathrm{W2o}\label{eq:dW_med/dt_full}
\end{split}\\
\begin{split}
%dovf/dt 
\frac{\mathrm{d}W_\mathrm{ovf}}{\mathrm{d}t}
&= \phi_\mathrm{W1o}
+ \phi_\mathrm{W2o}
- k_\mathrm{u_W}u_\mathrm{W3}\label{eq:dW_ovf/dt}
+ \phi_\mathrm{W_{cond}}
\end{split}\\
\begin{split}
\frac{\mathrm{d}B}{\mathrm{d}t} 
&=k_\mathrm{\alpha,\beta} \phi_\mathrm{C_{c\_p}}
- k_\mathrm{B_{p\_c}} \phi_\mathrm{C_{p\_c}}
\label{eq:dB/dt} 
\end{split}
\end{align}
\end{subequations}


The system under study is of the form:
\begin{align*}\label{eq:sys}
\mathbf{\dot{x}} &= \mathbf{f}(\mathbf{x}, \mathbf{u}, \mathbf{d}),
%\mathbf{y} &= \mathbf{x},
\end{align*}
with the state vector $\mathbf{x}=\mathbf{x}(t)$, output vector $\mathbf{y}=\mathbf{y}(t)$, input vector $\mathbf{u}=\mathbf{u}(t)$ and disturbance vector $\mathbf{d}=\mathbf{d}(t)$ given as
\begin{equation*}
\mathbf{x}= 
\begin{bmatrix} T \\
C\\
H\\
W_\mathrm{sto}\\
W_\mathrm{med}\\
W_\mathrm{ovf}\\
B\\
\end{bmatrix}, \;
\mathbf{y}= 
\begin{bmatrix} T \\
C\\
H\\
\end{bmatrix}, \;
\mathbf{u}= 
\begin{bmatrix} u_\mathrm{T} \\
u_\mathrm{V}\\
u_\mathrm{H}\\
u_\mathrm{W1}\\
u_\mathrm{W2}\\
u_\mathrm{W3}\\
u_{\mathrm{I}1}\\
u_{\mathrm{I}2}\\
u_{\mathrm{I}3}\\
u_{\mathrm{I}4}\\
\end{bmatrix}, \;
\mathbf{d}= 
\begin{bmatrix} T_\mathrm{out} \\
C_\mathrm{out}\\
H_\mathrm{out}\\
%I_\mathrm{out}\\
\end{bmatrix}. 
\end{equation*}
Constraints of the actuators, due to their construction, are given by
\begin{align*}
u_\mathrm{T} &\in[-100,100]\\
u_{\mathrm{I}i} &\in[0,100]\\
u_\mathrm{V},u_\mathrm{H},u_\mathrm{W1},u_\mathrm{W2},u_\mathrm{W3} &\in\{0,1\}
\end{align*}
which for brevity are combined into the constraint set $\mathbb{U} \subset \mathbb{R}^{10}$.
